SolO campfires in SDO images

I present the appearance of "Solar Orbiter campfires" in simultaneous images from the Solar Dynamics Observatory where most are visible although less sharp. I also show such features elsewhere in the SDO database. I show some in detail and discuss their nature.

==> figures.tex <==
%% file: figures.tex = temporarily separate for ease
%% init: Aug 10 2020  Rob Rutten  Deil from rebcontrails
%% last: Dec 16 2020  Rob Rutten  Deil
%% note: cp *ps from pertinent figsdir
%%       pspdfall   %% crops also
%%       pspdfallbb 27 35 241 243 field" to avoid label jumps (GONG)
%%       rm -f *ps


%% fig:soloim
%===========================================================================
\begin{figure*}
  \centering
  \includegraphics[width=\textwidth]{\deffigs/solorotim}
  \caption[Press-release SolO 174\,\AA\ image]{%
  \mbox{}\label{fig:soloim}   %RR must be here, not above figure (misfired)
  \addtocline{SolO press-release image} 
  Press-release SolO 174\,\AA\
  image, roughly rotated to solar $(X,Y)$ as seen from SDO. 
  After my long search for it this scene is burned into my brain.
  ``SolO campfires'' appear as tiny bright stalks; zoom-in may help to
  spot them. 
  It is the sole SolO input for this report; all other images are from
  SDO, plus one GONG \Halpha\ image. \\
  % No axes because location, scale and orientation remain
  % unspecified.\\
  {\bf Caveat disclaimer:} EUI PI David Berghmans reprimanded me later
  that this image ``is not properly validated'' and showing it here is
  ``unfair to the intrinsic quality of the EUI instrument'' -- but it
  serves here only to display the ``campfires'' shown and advertised
  during the SolO press conference, and as proof that I eventually did
  find this non-specified SolO scene in SDO (compare with
  \rrref{figure}{fig:field193}). 
  Proper validation may make this image yet better and enable proper
  axes, but will not affect any other image here nor SDO campfires in
  these (which by existing guarantee that the SolO ones can't validate
  away).\\
  {\em Copyright\/}: Solar Orbiter/EUI Team/ESA \& NASA; CSL, IAS, MPS,
  PMOD/WRC, ROB, UCL/MSSL.
  }\end{figure*}
%===========================================================================

%% ############## full-disk SDOs at best match-time

%% fig:fullmag
%===========================================================================
\begin{figure*}
  \centering
  \includegraphics[width=\textwidth]{\deffigs/sdo_full_magnetogram}
  \caption[Full-disk HMI magnetogram]{\label{fig:fullmag} %
  \addtocline{SDO SolO field}
  HMI magnetogram at best-match time, with the selected field marked
  by the white frame. 
  It contains the SolO field. 
  It did not contain major activity, present here only towards the
  East limb (where IRIS pointed that day, still farside for SolO).
  }\end{figure*}
%===========================================================================
%% fig:full1600
%===========================================================================
\begin{figure*}
  \centering
  \includegraphics[width=\textwidth]{\deffigs/sdo_full_1600}
  \caption[Full-disk AIA 1600\,\AA\ image]{\label{fig:full1600} %
  AIA 1600\,\AA\ image at best-match time. 
  It outlines the magnetic network seen in \rrref{figure}{fig:fullmag}
  very well as small bright grains obeying \rrref{figure}{fig:uvcartoons}.
  }\end{figure*}
%===========================================================================
%% fig:full304
%===========================================================================
\begin{figure*}
  \centering
  \includegraphics[width=\textwidth]{\deffigs/sdo_full_304}
  \caption[Full-disk AIA 304\,\AA\ image]{\label{fig:full304} AIA
  304\,\AA\ image at best-match time. 
  The dense coverage by grey patches is addressed in
  \rrref{appendix}{sec:ha304}. 
  They show the chromosphere with traditional ``transition region''
  temperatures but also visible in \Halpha. 
  Notice small brighter patches called ``brushfires'' below, as coyly
  as ``campfires'' but with language correction from Ron Moore
  (\rrref{footnote}{foot:moore}). 
  }\end{figure*}
%===========================================================================
%% fig:full171
%===========================================================================
\begin{figure*}
  \centering
  \includegraphics[width=\textwidth]{\deffigs/sdo_full_171}
  \caption[Full-disk AIA 171\,\AA\ image]{\label{fig:full171} %
  AIA 171\,\AA\ image at best-match time. 
  Obviously this AIA diagnostic is the best to show coronal
  connectivity and non-nearby-connectivity in polar plumes.
  }\end{figure*}
%===========================================================================
%% fig:full193
%===========================================================================
\begin{figure*}
  \centering
  \includegraphics[width=\textwidth]{\deffigs/sdo_full_193}
  \caption[Full-disk AIA 193\,\AA\ image]{\label{fig:full193} %
  AIA 193\,\AA\ image at best-match time. 
  This AIA diagnostic also shows coronal connectivity but outlines
  coronal holes (here especially at the poles) and similar areas of
  less optical thickness in hot coronal emissivity clearer.
  ``Fires'' (campfires or brushfires) stand out very well.  
  If you blur your vision the pattern within the box and the scene in
  \rrref{figure}{fig:soloim} agree, demonstrating that I did find the
  latter in SDO images -- eventually. 
  In hindsight, I mistakenly searched AIA 171\,\AA\ movies that looked
  as the preceding figure; with this diagnostic I might have succeeded
  faster.
  }\end{figure*}
%===========================================================================


%% ############### all SDO best-match full-field images

%% !! all need "pspdfallbb 27 35 241 243 field" or GONG jumps

%% fig:fieldmag
%===========================================================================
\begin{figure*}
  \centering
  \includegraphics[width=\textwidth]{\deffigs/field_hmimag}
  \caption[SolO-field HMI magnetogram]{\label{fig:fieldmag} %
  The SDO field at best-match time in the downloaded HMI magnetogram
  sequence.
  The greyscale is clipped at apparent flux density
  $B_{\rm app}^{\rm HMI} = \pm 200$~Mx\,cm$^{-2}$ to enhance the
  visibility of the network fields occupying this quiet area. 
  The subscript {\em app\/} stands for ``apparent'' following
  \citetads{1999ApJ...517.1013L} % Lites+Rutten+Berger H2v grains nonmagnetic
  to emphasize that while these units formally equal Gauss units, the
  actual intrinsic field strength in the magnetic concentrations (MC)
  charted here is much higher, of kilogauss amplitude. 
  The superscript {\em HMI\/} specifies the apparent/intrinsic ratio
  as a specific instrument property. 
  The small black and white (``bipolar'') MCs are roughly arranged in
  the apparent ``network'' incompletely outlining supergranular
  convection cells (\eg\
  \citeads{1997ApJ...487..424S}). % Schrijver++ sustaining network
  The grey internetwork in between shows just noise due to low
  sensitivity. 
  Charting internetwork fields needs higher sensitivity, as with
  Hinode/SP (\eg\
  \citeads{2008ApJ...672.1237L}). % Lites++ Hinode hor IN fields
  The area is quiet and generally mixed-polarity. 
  On small scales there appear to be many monopolar clusters of a
  dozen or so same-color grains, but with better magnetic sensitivity
  these likely will show opposite-polarity concentrations as well.
  In higher resolution observations all such MCs are no longer
  pointlike but have fast-varying morphology following local
  intergranular-lane dynamics (\eg\ the SST ``flowers'' of
  \citeads{2004A&A...428..613B}). % Berger++ SST flowers
  }\end{figure*}
%===========================================================================
%% fig:field1700
%===========================================================================
\begin{figure*}
  \centering
  \includegraphics[width=\textwidth]{\deffigs/field_aia1700}
  \caption[SolO-field AIA 1700\,\AA\ image]{\label{fig:field1700} %
  The SDO field at best-match time in the AIA 1700\,\AA\ image.
  The greyscale shows the square root of the intensity after clipping
  the brightest pixels in the 15-min sequence. 
  The scene shows ``bright points'' closely corresponding to the
  MCs in the preceding figure and roughly arranged in quasi-cellular
  supergranulation-driven network patterns with greyish internetwork
  shock interference patterns inside. 
  When playing the sequence as a movie the bright points remain fairly
  stationary while the shock patterns move around very fast in erratic
  fashion. 
  The latter are not discussed here but were brilliantly identified by
  \citetads{1997ApJ...481..500C} % Carlsson+Stein H2v grain simulation
  as clapotispheric shocks
  (\linkadspage{1995ESASP.376a.151R}{8}{Figure~12} of
  \citeads{1995ESASP.376a.151R}) % Rutten Asilomar %%RR why no ADS in refs?
  driven and patterned by $p$-mode interference.
  }\end{figure*}
%===========================================================================
%% fig:field1600
%===========================================================================
\begin{figure*}
  \centering
  \includegraphics[width=\textwidth]{\deffigs/field_aia1600}
  \caption[SolO-field AIA 1600\,\AA\ image]{\label{fig:field1600} %
  The SDO field at best-match time in the AIA 1600\,\AA\ image.
  The greyscale shows the square root of the intensity after clipping
  the brightest pixels in the 15-min sequence.
  The scene is very similar to the one in the 1700\,\AA\ image in
  preceding \rrref{figure}{fig:field1700}, but in blinking at sufficient
  zoom-in the 1600\,\AA\ bright points appear shifted limbward with
  different morphology. 
  This is detailed in \rrref{appendix}{sec:shift} and in
  \rrref{figure}{fig:uvcartoons} with a review-style caption.
  }\end{figure*}
%===========================================================================
%% fig:fieldha
%===========================================================================
\begin{figure*}
  \centering
  \includegraphics[width=\textwidth]{\deffigs/field_gongha}
  \caption[SolO-field in GONG \Halpha\ image] {\label{fig:fieldha} %
  The SDO field at best-match time in a simultaneous Big Bear GONG
  \Halpha\ image. %RR hopefully the best
  The cutout is bytescaled after severe clipping and limb darkening
  removal. 
  The angular resolution is too low to show that the darker, roughly
  linear, patches are made up of fibrils. 
  Higher-resolution \Halpha\ imaging would show that these emanate
  from network. 
  Yet-higher-resolution outer-wing \Halpha\ imaging would show slender
  recurrent RBEs and RREs emanating further from network
  (\linkadspage{2013ApJ...769...44S}{6}{Figure~4} of
  \citeads{2013ApJ...769...44S}). % Sekse RREs and RBEs
  \rrref{Appendix}{sec:ha304} argues that the latter produce the former.
  The plans for a DOT-clone GONG successor
  (\linkadspage{2019BAAS...51g..74H}{8}{Fig.~13} of
  \citeads{2019BAAS...51g..74H}) % Hill++ ngGONG white paper
  include \Halpha\ tuning to the outer wings.
  The present GONG network takes full-disk images of this quality
  sampling the wide core of \Halpha\ at 20\,s or slower cadence with
  24/7 coverage about 90\% since 2009, before SDO.
  The resolution is nominally twice worse but worsens further by
  station-dependent and time-dependent seeing also causing
  rubber-sheet warping. 
  See the \href{https://nso.edu/data/nisp-data/h-alpha}{GONG \Halpha\
  fact sheet}.
  }\end{figure*}
%===========================================================================
%% fig:fieldharev
%===========================================================================
\begin{figure*}
  \centering
  \includegraphics[width=\textwidth]{\deffigs/field_gongha_rev}
  \caption[SolO-field in reversed GONG \Halpha\ image]
  {\label{fig:fieldharev} %
  The same GONG \Halpha\ image as in preceding
  \rrref{figure}{fig:fieldha}, but with the greyscale reversed.
  This image is inserted here to facilitate blinking to the next (AIA
  304\,\AA). 
  How to blink pdf pages in a pdf reader is treated on
  \rrref{page}{sec:blinking}. 
  When you blink them the scenes appear to jump due to your eye
  detecting patch size differences but they are actually well aligned.
  This comparison is striking and discussed in \rrref{appendix}{sec:ha304}.
  }\end{figure*}
%===========================================================================
%% fig:field304
%===========================================================================
\begin{figure*}
  \centering
  \includegraphics[width=\textwidth]{\deffigs/field_aia304}
  \caption[SolO-field AIA 304\,\AA\ image]{\label{fig:field304} %
  The SDO field at best-match time in the AIA 304\,\AA\ image.
  The greyscale shows the logarithm of the intensity in rescaling with
  \href{https://webspace.science.uu.nl/~rutte101/rridl/sdolib/sdo_intscale.pro}{\tt
  sdo\_intscale.pro} and clipping the brightest pixels in the 15-min
  sequence. 
  Unfortunately, the AIA 304\,\AA\ channel lost much sensitivity over
  the years; initially the signal-to-noise was much better. 
  The campfires detailed in \rrref{section}{sec:campfires} are not very
  obvious but blinking against the next images shows they are here
  too. 
  Their presence here and in the next AIA 131\,\AA\ image led to the
  SDO fire detector defined in \rrref{figure}{fig:sdoroiloc304x131} and
  shown as second member in the triples of
  \rrref{figures}{fig:sdo-minx-193}--\ref{fig:sdo-sp-min-mag}.
  The brighter patches mark brushfires (\rrref{section}{sec:brushfires})
  that are also seen better in the next images. 
  Blinking back to the preceding reversed \Halpha\ image in
  \rrref{figure}{fig:fieldharev} shows rough but remarkable overall
  pattern correspondences everywhere for the grainy grey chromosphere
  patches.
  This similarity is discussed in \rrref{appendix}{sec:ha304}.
  }\end{figure*}
%===========================================================================
%% fig:field131
%===========================================================================
\begin{figure*}
  \centering
  \includegraphics[width=\textwidth]{\deffigs/field_aia131}
  \caption[SolO-field AIA 131\,\AA\ image]{\label{fig:field131} %
  The SDO field at best-match time in the AIA 131\,\AA\ image.
  The greyscale shows the logarithm of the intensity in rescaling with
  \href{https://webspace.science.uu.nl/~rutte101/rridl/sdolib/sdo_intscale.pro}{\tt
  sdo\_intscale.pro} and clipping the brightest pixels in the 15-min
  sequence. 
  This image is also noisy because the scene is so quiet, but it shows
  strict grey-patch correspondence with AIA 304\,\AA\ when blinking
  against preceding \rrref{figure}{fig:field304}, plus more diffuse
  brightenings that are clearer and more extended in the next AIA
  171\,\AA\ image. 
  Some campfires already stand out as tiny bright features.
  In \rrref{figure}{fig:sdoroiloc304x131} this image is multiplied with
  the preceding 304\,\AA\ image to demonstrate feasibility of global
  SDO fire detection.
  }\end{figure*}
%===========================================================================
% fig:field171
%===========================================================================
\begin{figure*}
  \centering
  \includegraphics[width=\textwidth]{\deffigs/field_aia171}
  \caption[SolO-field AIA 171\,\AA\ image]{\label{fig:field171} %
  The SDO field at best-match time in the AIA 171\,\AA\ image.
  The greyscale shows the logarithm of the intensity in rescaling with
  \href{https://webspace.science.uu.nl/~rutte101/rridl/sdolib/sdo_intscale.pro}{\tt
  sdo\_intscale.pro} and clipping the brightest pixels in the
  15-min sequence. 
  Blinking against the 131\,\AA\ scene in \rrref{figure}{fig:field131}
  shows addition of diffuse coronal connections. 
  I expected this image to be the one to be compared to the SolO
  press-release  174\,\AA\ image in \rrref{figure}{fig:soloim}.
  They cannot be blinked directly because they differ much in
  foreshortening, but the target scene is indeed the same.
  Actually the next one suits better. 
  }\end{figure*}
%===========================================================================
% fig:field193
%===========================================================================
\begin{figure*}
  \centering
  \includegraphics[width=\textwidth]{\deffigs/field_aia193}
  \caption[SolO-field AIA 193\,\AA\ image]{\label{fig:field193} %
  The SDO field at best-match time in the AIA 193\,\AA\ image.
  The greyscale shows the logarithm of the intensity in rescaling with
  \href{https://webspace.science.uu.nl/~rutte101/rridl/sdolib/sdo_intscale.pro}{\tt
  sdo\_intscale.pro} and clipping the brightest pixels in the 15-min
  sequence. 
  It shows yet more hazy coronal connectivity than the 171\,\AA\ image
  in preceding \rrref{figure}{fig:field171}.
  The tiny campfires stand out brightly where they occur in dark
  areas. 
  This image shows the best correspondence with the input
  press-release scene in \rrref{figure}{fig:soloim}, perhaps through
  the common high-intensity tails in next \rrref{figure}{fig:hists}.
  The larger bright patches are treated as brushfires in
  \rrref{section}{sec:brushfires}. 
  They represent classical coronal bright points (review by
  \citeads{2019LRSP...16....2M}). % Madjarska coronal BPs
  They are smaller and more homogeneously bright than in 171 and
  131\,\AA\ where they partly contain darker fibrils between brighter
  feet.
  }\end{figure*}
%===========================================================================


%% ########## fig:imhists
%===========================================================================
\begin{figure*}
  \centering
  \includegraphics[width=8cm]{\deffigs/hist-solo}
  \includegraphics[width=8cm]{\deffigs/hist-sdo-171}\\
  \includegraphics[width=8cm]{\deffigs/hist-sdo-131}
  \includegraphics[width=8cm]{\deffigs/hist-sdo-193}
  \caption[Pixel intensity histograms]{\label{fig:hists} %
  Histograms of the pixel intensities in the SolO 174\,\AA\ image and
  in three SDO images at the best-match time, respectively SDO
  171\,\AA, 131\,\AA\ and 193\,\AA. 
  Extended highest-brightness tails show up in all but especially in
  the SolO 174\,\AA\ and AIA 193\,\AA\ distributions. 
  The latter also shows a double-hump peak; there are indeed many dark
  areas in \rrref{figure}{fig:field193}.
  }\end{figure*}
%===========================================================================


%% ################### other quadrants and years

% fig:sdo-minx-193
%===========================================================================
\begin{figure*}
  \centering
  \includegraphics[width=\textwidth]{\deffigs/sdo-minx_193}
  \caption[AIA 193\,\AA\ image in the North-East]
  {\label{fig:sdo-minx-193} %
  \addtocline{SDO other-field triples} Comparable AIA 193\,\AA\ cutout
  for May 30, 2020 14:58:46~UT as in \rrref{figure}{fig:field193} but
  East at $(X,Y) = (-375,148)$.
  Just as the SolO field this same-size other field shows about a
  dozen tiny campfires and more larger brushfires.
  Wider-connecting diffuse 193\,\AA\ brightness patterns occur mostly
  around brushfires and suggest origin in earlier or persistent
  brushfires. 
  }\end{figure*}
%===========================================================================
% fig:sdo-minx-fire
%===========================================================================
\begin{figure*}
  \centering
  \includegraphics[width=\textwidth]{\deffigs/sdo-minx_304x131}
  \caption[SDO fire detector in the North-East]
  {\label{fig:sdo-minx-fire} %
  SDO fire detector cutout for the same field as in preceding
  \rrref{figure}{fig:sdo-minx-193}.
  Its construction is described in the caption of
  \rrref{figure}{fig:sdoroiloc304x131}.
  It serves to separate chromospheric heating (ubiquitous grey
  patches) and coronal heating (small dispersed areas colored cyan).
  In these and the following ``other SDO scene'' triples these fire
  detector images are inserted between the AIA 193\,\AA\ images and
  the HMI magnetograms for blinking backward and forward with these.
  It shows that many small bright 193\,\AA\ loop bundles
  constituting larger brushfires have cyan-colored detector
  brightenings at their feet located in bipolar network.
  The smallest point-like campfires go without such closed-loop
  connectivity.
  }\end{figure*}
%===========================================================================
% fig:sdo-minx-mag
%===========================================================================
\begin{figure*}
  \centering
  \includegraphics[width=\textwidth]{\deffigs/sdo-minx_mag}
  \caption[HMI magnetogram in the North-East]
  {\label{fig:sdo-minx-mag} %
  HMI magnetogram for the field in the two preceding figures.
  The field strengths are clipped as described for
  \rrref{figure}{fig:fieldmag}.
  Blinking with the two preceding figures shows that small
  ``brushfire'' loop bundles in 193\,\AA\ connect small groups of
  opposite-polarity MCs.
  }\end{figure*}
%===========================================================================

% fig:sdo-miny-193
%===========================================================================
\begin{figure*}
  \centering
  \includegraphics[width=\textwidth]{\deffigs/sdo-miny_193}
  \caption[AIA 193\,\AA\ image in the South-West]
  {\label{fig:sdo-miny-193} %
  Comparable AIA 193\,\AA\ cutout for May 30, 2020 14:58:46~UT T as in
  \rrref{figure}{fig:field193} but South at $(X,Y) = (375,-148)$.
  Again about a dozen tiny campfires and more larger brushfires.
  }\end{figure*}
%===========================================================================
% fig:sdo-miny-fire
%===========================================================================
\begin{figure*}
  \centering
  \includegraphics[width=\textwidth]{\deffigs/sdo-miny_304x131}
  \caption[SDO fire detector image in the South-West]
  {\label{fig:sdo-miny-fire} %
  SDO fire detector cutout for the same field as in preceding
  \rrref{figure}{fig:sdo-miny-193}.
  }\end{figure*}
%===========================================================================
% fig:sdo-miny-mag
%===========================================================================
\begin{figure*}
  \centering
  \includegraphics[width=\textwidth]{\deffigs/sdo-miny_mag}
  \caption[HMI magnetogram in the South-West]
  {\label{fig:sdo-miny-mag} %
  HMI magnetogram for the field in the two preceding figures.
  }\end{figure*}
%===========================================================================
 
% fig:sdo-minx-miny-193
%===========================================================================
\begin{figure*}
  \centering
  \includegraphics[width=\textwidth]{\deffigs/sdo-minx-miny_193}
  \caption[AIA 193\,\AA\ image in the South-East]
{\label{fig:sdo-minx-miny-193} %
  Comparable AIA 193\,\AA\ cutout for May 30, 2020 14:58:46~UT as in
  \rrref{figure}{fig:field193} but South-East at $(X,Y) = (-375,-148)$.
  }\end{figure*}
%===========================================================================
% fig:sdo-minx-miny-fire
%===========================================================================
\begin{figure*}
  \centering
  \includegraphics[width=\textwidth]{\deffigs/sdo-minx-miny_304x131}
  \caption[SDO fire detector image in the South-East]
  {\label{fig:sdo-minx-miny-fire} %
  SDO fire detector cutout for the same field as in the preceding
  figure.  
  Around the small active plage at lower-left some campfires are
  veiled by coronal loops in the preceding AIA 193\,\AA\ image
  put appear unveiled in this chart.
  }\end{figure*}
%===========================================================================
% fig:sdo-minx-miny-mag
%===========================================================================
\begin{figure*}
  \centering
  \includegraphics[width=\textwidth]{\deffigs/sdo-minx-miny_mag}
  \caption[HMI magnetogram in the South-East]
  {\label{fig:sdo-minx-miny-mag} %
  HMI magnetogram for the field in the two preceding figures.
  }\end{figure*}
%===========================================================================

%% ####### other years same location 

% fig:sdo2019_193
%===========================================================================
\begin{figure*}
  \centering
  \includegraphics[width=\textwidth]{\deffigs/sdo2019_193}
  \caption[SolO-field AIA 193\,\AA\ image in 2019]
  {\label{fig:sdo2019-193} %
  Comparable AIA 193\,\AA\ cutout for the same $(X,Y) = (375,148)$
  arcsec location as best-match \rrref{figure}{fig:field193} and also
  on May 30 near 14:58~UT, but in 2019. 
  There is a small active plage near the center.
  }\end{figure*}
%===========================================================================
% fig:sdo2019-fire
%===========================================================================
\begin{figure*}
  \centering
  \includegraphics[width=\textwidth]{\deffigs/sdo2019_304x131}
  \caption[SolO-field SDO fire detector image in 2019]
  {\label{fig:sdo2019-fire} %
  SDO fire detector cutout for the same field as in the preceding
  figure.
  }\end{figure*}
%===========================================================================
% fig:sdo2019-mag
%===========================================================================
\begin{figure*}
  \centering
  \includegraphics[width=\textwidth]{\deffigs/sdo2019_mag}
  \caption[SolO-field HMI magnetogram in 2019]
  {\label{fig:sdo2019-mag} %
  HMI magnetogram for the field in the two preceding figures.
  }\end{figure*}
%===========================================================================

% fig:sdo2018_193
%===========================================================================
\begin{figure*}
  \centering
  \includegraphics[width=\textwidth]{\deffigs/sdo2018_193}
  \caption[SolO-field AIA 193\,\AA\ image in 2018]
  {\label{fig:sdo2018-193} %
  Comparable AIA 193\,\AA\ cutout for the same $(X,Y) = (375,148)$
  arcsec location as best-match \rrref{figure}{fig:field193} and also on
  May 30 near 14:58~UT, but in 2018. 
  This scene is the most active portrayed in this report. 
  }\end{figure*}
%===========================================================================
% fig:sdo2018-fire
%===========================================================================
\begin{figure*}
  \centering
  \includegraphics[width=\textwidth]{\deffigs/sdo2018_304x131}
  \caption[SolO-field SDO fire detector image in 2018]
  {\label{fig:sdo2018-fire} %
  SDO fire detector cutout for the same field as in the preceding
  figure. 
  The bytescale is clipped for the active region to maintain visibilty
  (grey) of the quiet network elsewhere, as described under
  \rrref{figure}{fig:sdoroiloc304x131}.
  }\end{figure*}
%===========================================================================
% fig:sdo2018-mag
%===========================================================================
\begin{figure*}
  \centering
  \includegraphics[width=\textwidth]{\deffigs/sdo2018_mag}
  \caption[SolO-field HMI magnetogram in 2018]
  {\label{fig:sdo2018-mag} %
  HMI magnetogram for the field in the two preceding figures.
  }\end{figure*}
%===========================================================================

% fig:sdo2017_193
%===========================================================================
\begin{figure*}
  \centering
  \includegraphics[width=\textwidth]{\deffigs/sdo2017_193}
  \caption[SolO-field AIA 193\,\AA\ image in 2017]
  {\label{fig:sdo2017-193} %
  Comparable AIA 193\,\AA\ cutout for the same $(X,Y) = (375,148)$
  arcsec location as best-match \rrref{figure}{fig:field193} and also on
  May 30 near 14:58~UT, but in 2017.
  }\end{figure*}
%===========================================================================
% fig:sdo2017-fire
%===========================================================================
\begin{figure*}
  \centering
  \includegraphics[width=\textwidth]{\deffigs/sdo2017_304x131}
  \caption[SolO-field SDO fire detector image in 2017]
  {\label{fig:sdo2017-fire} %
  SDO fire detector cutout for the same field as in the preceding
  figure.
  }\end{figure*}
%===========================================================================
% fig:sdo2017-mag
%===========================================================================
\begin{figure*}
  \centering
  \includegraphics[width=\textwidth]{\deffigs/sdo2017_mag}
  \caption[SolO-field HMI magnetogram in 2017]
  {\label{fig:sdo2017-mag} %
  HMI magnetogram for the field in the two preceding figures.
  The small active region is mostly monopolar but at higher
  sensitivity than offered by HMI it is rather likely that there are
  or have been canceling white-polarity MCs.
  }\end{figure*}
%===========================================================================

%% ##### poles max and min

% fig:sdo-np-max_193
%===========================================================================
\begin{figure*}
  \centering
  \includegraphics[width=\textwidth]{\deffigs/sdo-np-max_193}
  \caption[North-pole AIA 193\,\AA\ image at maximum]
  {\label{fig:sdo-np-max-193} %
  AIA 193\,\AA\ cutout near the solar North pole on April 1, 2014 at
  00:00~UT. 
  Much activity at lower latitudes.
  }\end{figure*}
%===========================================================================
% fig:sdo-np-max-fire
%===========================================================================
\begin{figure*}
  \centering
  \includegraphics[width=\textwidth]{\deffigs/sdo-np-max_304x131}
  \caption[North-pole SDO fire detector image at maximum]
  {\label{fig:sdo-np-max-fire} %
  SDO fire detector cutout for the same field as in the preceding
  figure. 
  There are very few fires here in the upper part North of the active
  regions. 
  All the grey chromosphere patches suggest more. 
  I wonder whether you must look down their throat to see them.  
  I applied ${\tt heightdiff} = 1000$~km correction (see
  \rrref{appendix}{sec:16001700}) to the whole field but this made no
  difference. 
  There may also be too much veiling along the slanted lines of sight
  by all the widely-connected coronal haze in the preceding figure.
  }\end{figure*}
%===========================================================================
% fig:sdo-np-max-mag
%===========================================================================
\begin{figure*}
  \centering
  \includegraphics[width=\textwidth]{\deffigs/sdo-np-max_mag}
  \caption[North-pole HMI magnetogram at maximum]
  {\label{fig:sdo-np-max-mag} %
  HMI magnetogram for the field in the two preceding figures.
  }\end{figure*}
%===========================================================================

% fig:sdo-np-min-193
%===========================================================================
\begin{figure*}
  \centering
  \includegraphics[width=\textwidth]{\deffigs/sdo-np-min_193}
  \caption[North-pole AIA 193\,\AA\ image at minimum]
  {\label{fig:sdo-np-min-193} %
  AIA 193\,\AA\ cutout near the solar North pole on June 1,2019 at
  00:00~UT. 
  }\end{figure*}
%===========================================================================
% fig:sdo-np-min-fire
%===========================================================================
\begin{figure*}
  \centering
  \includegraphics[width=\textwidth]{\deffigs/sdo-np-min_304x131}
  \caption[North-pole SDO fire detector image at minimum]
  {\label{fig:sdo-np-min-fire} %
  SDO fire detector cutout for the same field as in the preceding
  figure. 
  The small-fire density is much higher than in maximum-activity
  \rrref{figure}{fig:sdo-np-max-fire}.
  }\end{figure*}
%===========================================================================
% fig:sdo-np-min-mag
%===========================================================================
\begin{figure*}
  \centering
  \includegraphics[width=\textwidth]{\deffigs/sdo-np-min_mag}
  \caption[North-pole HMI magnetogram at minimum]
  {\label{fig:sdo-np-min-mag} %
  HMI magnetogram for the field in the two preceding figures.
  }\end{figure*}
%===========================================================================

% fig:sdo-sp-max_193
%===========================================================================
\begin{figure*}
  \centering
  \includegraphics[width=\textwidth]{\deffigs/sdo-sp-max_193}
  \caption[South-pole AIA 193\,\AA\ image at maximum]
  {\label{fig:sdo-sp-max-193} %
  AIA 193\,\AA\ cutout near the solar South pole on April 1, 2014 at
  00:00~UT.
  }\end{figure*}
%===========================================================================
% fig:sdo-sp-max-fire
%===========================================================================
\begin{figure*}
  \centering
  \includegraphics[width=\textwidth]{\deffigs/sdo-sp-max_304x131}
  \caption[South-pole SDO fire detector image at maximum]
  {\label{fig:sdo-sp-max-fire} %
  SDO fire detector cutout for the same field as in the preceding
  figure. 
  High fire warning, less in the polar hole.
  }\end{figure*}
%===========================================================================
% fig:sdo-sp-max-mag
%===========================================================================
\begin{figure*}
  \centering
  \includegraphics[width=\textwidth]{\deffigs/sdo-sp-max_mag}
  \caption[South-pole HMI magnetogram at maximum]
  {\label{fig:sdo-sp-max-mag} %
  HMI magnetogram for the field in the two preceding figures.
  }\end{figure*}
%===========================================================================

% fig:sdo-sp-min_193
%===========================================================================
\begin{figure*}
  \centering
  \includegraphics[width=\textwidth]{\deffigs/sdo-sp-min_193}
  \caption[South-pole AIA 193\,\AA\ image at minimum]
  {\label{fig:sdo-sp-min-193} %
  AIA 193\,\AA\ cutout near the solar South pole on June 1, 2019 at
  00:00~UT.
  }\end{figure*}
%===========================================================================
% fig:sdo-sp-min-fire
%===========================================================================
\begin{figure*}
  \centering
  \includegraphics[width=\textwidth]{\deffigs/sdo-sp-min_304x131}
  \caption[South-pole SDO fire detector at minimum]
  {\label{fig:sdo-sp-min-fire} %
  SDO fire detector cutout for the same field as in the preceding
  figure.
  }\end{figure*}
%===========================================================================
% fig:sdo-sp-min-mag
%===========================================================================
\begin{figure*}
  \centering
  \includegraphics[width=\textwidth]{\deffigs/sdo-sp-min_mag}
  \caption[South-pole HMI magnetogram at minimum]
  {\label{fig:sdo-sp-min-mag} %
  HMI magnetogram for the field in the two preceding figures.
  }\end{figure*}
%===========================================================================

\clearpage %RR otherwise too many floats for latex



%% ######## campfire ROI figures, first ROI locations in SolO image

% fig:cfroilocs
%===========================================================================
\begin{figure*}
  \centering
  \includegraphics[width=\textwidth]{\deffigs/cfroiloc174}
  \caption[Campfire cutout locations in the SolO image]
  {\label{fig:cfroilocs} %
  \addtocline{SDO campfire ROI cutouts}
  The rotated SolO 174\,\AA\ image with superimposed ROI boxes for the
  campfire cutouts. 
  ROI-1 is the campfire that was marked in the annotated version in
  the press-release material.
  The others are eye-ball selected in top-to-bottom order, also
  including small bright patches with more complex than single-flame
  morphology.
  }\end{figure*}
%===========================================================================

%% ################ all ROI figs

%% fig:roi1
%===========================================================================
\begin{figure*}
  \centering
  \includegraphics[width=\textwidth]{\deffigs/cfroi1}
  \caption[ROI-1 cutout assembly]{\label{fig:roi1} %
  Cutouts for ROI-1. 
  Format details are given in the main text in
  \rrref{section}{sec:campfires}.
  This SolO campfire (top) was annotated as exemplary in the press
  release.
  It was also present in the AIA EUV images, also recurrently before,
  best in AIA 304\,\AA. 
  There was a bipolar MC pair on the surface underneath, with enhanced
  brightening in the UV including excess in the 16001700 construct. 
  }\end{figure*}
%===========================================================================
%% fig:roi2
%===========================================================================
\begin{figure*}
  \centering
  \includegraphics[width=0.97\textwidth]{\deffigs/cfroi2} %RR too high
  \caption[ROI-2 cutout assembly]{\label{fig:roi2} %
  Cutouts for ROI-2.
  }\end{figure*}
%===========================================================================
%% fig:roi3
%===========================================================================
\begin{figure*}
  \centering
 \includegraphics[width=\textwidth]{\deffigs/cfroi3}
  \caption[ROI-3 cutout assembly]{\label{fig:roi3} %
  Cutouts for ROI-3.
  }\end{figure*}
%===========================================================================
%% fig:roi4
%===========================================================================
\begin{figure*}
  \centering
  \includegraphics[width=\textwidth]{\deffigs/cfroi4}
  \caption[ROI-4 cutout assembly]{\label{fig:roi4} %
  Cutouts for ROI-4.
  }\end{figure*}
%===========================================================================
%% fig:roi5
%===========================================================================
\begin{figure*}
  \centering
  \includegraphics[width=\textwidth]{\deffigs/cfroi5}
  \caption[ROI-5 cutout assembly]{\label{fig:roi5} %
  Cutouts for ROI-5.
  }\end{figure*}
%===========================================================================
%% fig:roi6
%===========================================================================
\begin{figure*}
  \centering
  \includegraphics[width=\textwidth]{\deffigs/cfroi6}
  \caption[ROI-6 cutout assembly]{\label{fig:roi6} %
  Cutouts for ROI-6.
  }\end{figure*}
%===========================================================================
%% fig:roi7
%===========================================================================
\begin{figure*}
  \centering
  \includegraphics[width=\textwidth]{\deffigs/cfroi7}
  \caption[ROI-7 cutout assembly]{\label{fig:roi7} %
  Cutouts for ROI-7.
  }\end{figure*}
%===========================================================================
%% fig:roi8
%===========================================================================
\begin{figure*}
  \centering
  \includegraphics[width=\textwidth]{\deffigs/cfroi8}
  \caption[ROI-8 cutout assembly]{\label{fig:roi8} %
  Cutouts for ROI-8.
  }\end{figure*}
%===========================================================================
%% fig:roi9
%===========================================================================
\begin{figure*}
  \centering
  \includegraphics[width=\textwidth]{\deffigs/cfroi9}
  \caption[ROI-9 cutout assembly]{\label{fig:roi9} %
  Cutouts for ROI-9.
  }\end{figure*}
%===========================================================================
%% fig:roi10
%===========================================================================
\begin{figure*}
  \centering
  \includegraphics[width=\textwidth]{\deffigs/cfroi10}
  \caption[ROI-10 cutout assembly]{\label{fig:roi10} %
  Cutouts for ROI-10.
  }\end{figure*}
%===========================================================================
%% fig:roi11
%===========================================================================
\begin{figure*}
  \centering
  \includegraphics[width=\textwidth]{\deffigs/cfroi11}
  \caption[ROI-11 cutout assembly]{\label{fig:roi11} %
  Cutouts for ROI-11.
  }\end{figure*}
%===========================================================================
%% fig:roi12
%===========================================================================
\begin{figure*}
  \centering
  \includegraphics[width=\textwidth]{\deffigs/cfroi12}
  \caption[ROI-12 cutout assembly]{\label{fig:roi12} %
  Cutouts for ROI-12.
  }\end{figure*}
%===========================================================================

\clearpage %RR otherwise too many floats for latex

%% ######## brushfire ROI figures, first ROI locations in SolO image

% fig:bfroilocs
%===========================================================================
\begin{figure*}
  \centering
  \includegraphics[width=\textwidth]{\deffigs/bfroiloc174}
  \caption[Brushfire cutout locations in the SolO image]
  {\label{fig:bfroilocs} %
  The rotated SolO 174\,\AA\ image with superimposed ROI boxes for the
  brushfire cutouts. 
  }\end{figure*}
%===========================================================================

%% ################ brushfire ROI figs

%% fig:bfroiA
%==========================================================================
\begin{figure*}
  \centering
  \includegraphics[width=0.9\textwidth]{\deffigs/bfroi1}
  \caption[ROI-A cutout assembly]{\label{fig:roiA} %
  \addtocline{SDO brushfire ROI cutouts}
  Cutouts for ROI-A.  
  }\end{figure*}
%===========================================================================
%% fig:bfroiB
%===========================================================================
\begin{figure*}
  \centering
  \includegraphics[width=0.9\textwidth]{\deffigs/bfroi2}
  \caption[ROI-B cutout assembly]{\label{fig:roiB} %
  Cutouts for ROI-B.
  }\end{figure*}
%===========================================================================
%% fig:bfroiC
%===========================================================================
\begin{figure*}
  \centering
  \includegraphics[width=0.9\textwidth]{\deffigs/bfroi3}
  \caption[ROI-C cutout assembly]{\label{fig:roiC} %
  Cutouts for ROI-C.
  }\end{figure*}
%===========================================================================
%% fig:bfroiD
%===========================================================================
\begin{figure*}
  \centering
  \includegraphics[width=0.9\textwidth]{\deffigs/bfroi4}
  \caption[ROI-D cutout assembly]{\label{fig:roiD} %
  Cutouts for ROI-D.
  }\end{figure*}
%===========================================================================
%% fig:bfroiE
%===========================================================================
\begin{figure*}
  \centering
  \includegraphics[width=0.9\textwidth]{\deffigs/bfroi5}
  \caption[ROI-E cutout assembly]{\label{fig:roiE} %
  Cutouts for ROI-E.
  }\end{figure*}
%===========================================================================

% fig:sdoroilocmag
%===========================================================================
\begin{figure*}
  \centering
  \includegraphics[width=\textwidth]{\deffigs/sdoroilocmag}
  \caption[All cutouts in HMI magnetogram]
  {\label{fig:sdoroilocmag} %
  \addtocline{SDO ROI locations and fire detector}
  The HMI magnetogram at best-match time with superimposed ROI boxes
  for all campfire and brushfire cutouts.
  }\end{figure*}
%===========================================================================
% fig:sdoroiloc193
%===========================================================================
\begin{figure*}
  \centering
  \includegraphics[width=\textwidth]{\deffigs/sdoroiloc193}
  \caption[All cutouts in AIA 193\,\AA\ image]
  {\label{fig:sdoroiloc193} %
  The AIA 193\,\AA\ image at best-match time with superimposed ROI boxes
  for all campfire and brushfire cutouts.
  }\end{figure*}
%===========================================================================
% fig:sdoroiloc131
%===========================================================================
\begin{figure*}
  \centering
  \includegraphics[width=\textwidth]{\deffigs/sdoroiloc131}
  \caption[All cutouts in AIA 131\,\AA\ image]
  {\label{fig:sdoroiloc131} %
  The AIA 131\,\AA\ image at best-match time with superimposed ROI
  boxes for all campfire and brushfire cutouts.
  Green and blue pixels are those within the green and blue
  selection boxes in the righthand Strous diagram in
  \rrref{figure}{fig:scats}.
  Green pixels lie mostly in the bright patch in the
  lower-right corner;  blue pixels lie in small bright features.
  Blinking with the preceding AIA\,193\,\AA\ image shows that most
  are small brushfires, with bipolar MCs on the surface (blink
  one more back).  However, most campfires also contain blue pixels.
  These colored pixel selections inspired the next figure.
  }\end{figure*}
%===========================================================================
% fig:sdoroiloc304x131
%===========================================================================
\begin{figure*}
  \centering
  \includegraphics[width=\textwidth]{\deffigs/sdoroilocs_304x131}
  \caption[All cutouts in AIA 304$\times$131 construct]
  {\label{fig:sdoroiloc304x131} %
  SDO fire detector inspired by blinking AIA~304 and 131\,\AA\ in
  \rrref{figures}{fig:field304} and \ref{fig:field131}, {\tt EBFAF}
  detection (\rrref{appendix}{sec:ebfaf}) and by the blue pixels in
  the preceding figure selected with the blue box in
  \rrref{figure}{fig:scats}.
  The scene is a construct: the best-match AIA 304\,\AA\ image in
  \rrref{figure}{fig:field304} is multiplied by its 131\,\AA\
  companion in \rrref{figure}{fig:field131}.
  The check plot in \rrref{figure}{fig:drifts} for this pair shows
  that their alignment is sufficiently precise.
  The brightest product pixels are colored cyan, chosen to convey
  EUV-hot fire temperature. 
  The greyscale clip and color threshold are defined by the
  sequence-averaged quiet-network areas only, to avoid lopsiding by
  brighter active regions as present in
  \rrref{figure}{fig:sdo2018-fire}. 
  The values are determined in
  \href{https://webspace.science.uu.nl/~rutte101/rridl/sdolib/sdo_firelevel.pro}{\tt
  sdo\_firelevel.pro} by iteratively removing brightest pixels in
  average and rms computation for the full sequence.
  The values used here are 10\,$\sigma$ of left-over network above its
  average to clip active regions and
  4.5\,$\sigma$ threshold to color pixels cyan.\\
  This stringent pixel-value selection appears useful as EUV fire
  detector. 
  Spatial extent and temporal duration may then discriminate between
  small momentary campfires versus wider and more persistent
  brushfires. \\
  The grey patches everywhere else represent dynamic chromosphere
  around quiet network. 
  They are ubiquitously present with similar appearance in spreading
  around network MC concentrations, defining grey in this image
  well-suited as heated-chromosphere locator.
  It is hot since it is seen here and also as grey background in
  171\,\AA\ (\rrref{figure}{fig:field171}), AIA 221\,\AA\ and AIA
  335\,\AA, but it is also darkly visible in \Halpha\ (blink with
  \rrref{figure}{fig:fieldharev}).
  This dual visibility is discussed in \rrref{appendix}{sec:ha304}. \\
  The darkest patches between the grey ones generally match dark
  features present in most other AIA EUVs and seen sharpest in
  171\,\AA.
  However, in 193\,\AA\ (\rrref{figure}{fig:sdoroiloc193} or
  \rrref{figure}{fig:field193}) many seem covered by diffuse emission
  and others appear bright, for example the brushfire loop bundle to
  the right of ROI-A between ROI-3 and ROI-7 which only has footpoint
  pixels colored cyan here while most loops in this 193\,\AA-bright
  bundle appear dark in 131\,\AA\ (\rrref{figure}{fig:sdoroiloc131} or
  \rrref{figure}{fig:field131}) and in 171\,\AA\
  (\rrref{figure}{fig:field171}).
  Also this dual visibility is discussed in \rrref{appendix}{sec:ha304}.\\
  Ten other fire detector scenes are shown as triple member in
  \rrref{figures}{fig:sdo-minx-193}--\ref{fig:sdo-sp-min-mag}.  
  They separate well between chromospheric and coronal heating.
  }\end{figure*}
%===========================================================================

%% ################### 1600-1700 tileshift figures

% fig:tileshifts-1617-0
%===========================================================================
\begin{figure*}
  \centering
  \includegraphics[width=0.9\textwidth]{\deffigs/tileshifts-diff0}
  \caption[Tile shifts 1700--1600\,\AA] 
  {\label{fig:tileshifts-1617-0} %
  \addtocline{Appendix A}
  Vector chart of apparent shifts of features in AIA 1700\,\AA\ to
  their location in AIA 1600\,\AA, measured by cross-correlation per
  subfield tile at the best-match time. 
  The tiles are greyscaled to their vector length.  
  Similar radial-expansion charts result throughout the SDO database. 
  They represent my closest endeavor to cosmology.
  }\end{figure*}
%===========================================================================

% fig:zonalshifts-1617-0
%===========================================================================
\begin{figure*}
  \centering
  \includegraphics[width=0.6\textwidth]{\deffigs/zonalshifts-diff0}
  \caption[Zonal azimuthal tile-shift averages]
  {\label{fig:zonalshifts-1617-0} %
  Amplitudes of the shift vectors in
  \rrref{figure}{fig:tileshifts-1617-0} averaged azimuthally along
  circular zones.
  The lower curve is the zonal average for the radial components.
  I attribute the final uptilt to \CIV\ contribution in AIA 1600\,\AA\
  and chose ${\tt heightdiff} = 220$~km for
  \href{https://webspace.science.uu.nl/~rutte101/rridl/sdolib/sdo_muckimagepair.pro}{\tt
  sdo\_muckimagepair.pro} from this graph, in agreement with the
  measurement by
  \citetads{2019SoPh..294..161A}. % Alissandrakis AIA heights
  This value is not height-of-formation difference between samplings of
  vertical features as commonly thought, but a formal way of
  quantifying the apparent limbward displacements in
  \rrref{figure}{fig:tileshifts-1617-0}.
  Their actual cause is explained in \rrref{figure}{fig:uvcartoons}.
  }\end{figure*}
%===========================================================================

% fig:tileshifts-1617-220
%===========================================================================
\begin{figure*}
  \centering
  \includegraphics[width=0.9\textwidth]{\deffigs/tileshifts-diff220}
  \caption[Tile shifts 1700--1600\,\AA\ after {\tt heightdiff}]
  {\label{fig:tileshifts-1617-220} %
  Vector chart of apparent AIA 1700 to 1600\,\AA\ shifts after
  shift-back correction per tile using {\tt heightdiff} = 220~km as
  formal limb value.
  The vector scale is expanded 3.6~times compared with
  \rrref{figure}{fig:tileshifts-1617-0}.  
  I found closely similar residue patterns throughout the SDO database
  and do not understand it. 
  }\end{figure*}
%===========================================================================

% fig:uvcartoons
%===========================================================================
\begin{figure*}
  \centering
  \includegraphics[width=6cm]{\deffigs/G-form-radial} 
  \hspace{2cm}
  \includegraphics[width=6cm]{\deffigs/G-form-slant}\\[4ex]
  \includegraphics[width=6cm]{\deffigs/UV1617-center}
  \hspace{2cm}
  \includegraphics[width=6cm]{\deffigs/UV1617-slant}
  \caption[MC brightening at 1700 and 1600\,\AA] 
  {\label{fig:uvcartoons} %
  {\em Top row\/}: ancient sketches to explain G-band brightening of
  `''filigree grains'' (here called magnetic concentrations = MCs,
  also known as flux tubes, fluxtubes, magnetic elements, magnetic
  bright points, intergranular bright points, network points, facular
  points, faculae, plage, flowers, pseudo-EBs, line gaps,
  pseudo-moustaches) copied from
  \linkadspage{1999ASPC..184..181R}{8}{Figure 7} in
  \citetads{1999ASPC..184..181R}.\\ % Rutten Potsdam review
  {\em Left:\/} the radial view at disk center.  
  This cartoon was first drawn by Kees Zwaan, based on his
  thesis (\citeads{1965smss.book.....Z}) % Zwaan thesis
  and extract \citetads{1967SoPh....1..478Z}, % Zwaan: invisible sunspots
  much discussed at Sterrewacht Sonnenborgh (with Hans Rosenberg on
  this
  \href{https://webspace.science.uu.nl/~rutte101/astronomershots/album1967/kees-zwaan-hans-rosenberg.jpg}{1967
  photograph}), and finally published as
  \linkadspage{1978SoPh...60..213Z}{12}{Fig.~2} of
  \citetads{1978SoPh...60..213Z}. % Zwaan flux appearance
  The Zwaan-style fluxtube is relatively empty because its magnetic
  pressure compensates part of the outside gas pressure in
  magnetostatic equilibrium
  (\citeads{1976SoPh...50..269S}, % Spruit, magnetostatic fluxtube
  Zwaan-inspired in contrast to this
  \linkadspage{1990IAUS..138..501R}{10}{creation diagram}). 
  Zwaan's concept was observationally quantified by Sami Solanki and
  coworkers into Z\"urich wine-glass models (\eg\
  \citeads{1993A&A...268..736B}) % Bunte+Solank+Steiner wine glass
  using unresolved but sensitive multi-line spectropolarimetry
  initiated by \citetads{1984AdSpR...4h...5S} % Stenflo FTS multiline
  (see \citeads{1984A&A...131..333S}, % Stenflo++ FTS multiline
  \citeads{1993SSRv...63....1S}). %Solanki new testament
  The concept applies to gas-dominated atmospheric stratification with
  upward fluxtube flaring set by hydrostatic density decrease; for
  non-flaring field-dominated magnetostatic coronal loops see \eg\
  \citetads{1985ApJ...293...31L}, % BC Low magnetostatic
  \citetads{2004A&A...417..333N}.\\ % November magnetohydrostatic
  {\em Visibility:\/} top-down one views deeper into the fluxtube and
  receives larger brightness from its hotter hole-in-the-surface walls
  and bottom than from the field-free gas around it. 
  The latter is sampled higher at lower temperature and also in a
  relatively dark intergranular lane (so that at
  non-subarcsec resolution these small brightenings and their
  surroundings blend into non-showing grey,
  \citeads{1996ApJ...463..797T}). % Title+Berger G BP double Gaussare .
  In the G-band the low pressure causes extra dissociation of the CH
  molecules causing this Fraunhofer-named dark spectral feature, so
  that images selecting it show enhanced brightening compared to
  continuum wavelengths.   
  Because this band is wide enough to accommodate interference-filter
  10\,\AA\ bandpass it became very popular in short-exposure
  high-resolution photosphere imaging after
  \citetads{1984apoa.conf..382M} % Muller but no pdf, is this the CN one?
  did so first.
  Thus, MC brightening comes from holes in the surface, deeper in the
  G-band, not necessarily from extra heating.
  The \CaII\ \HK\ wing study of
  \citetads{2005A&A...437.1069S} % Sheminova++ catube
  found no MC heating throughout the photosphere, in conflict with the
  increasing temperature excess that is stipulated in plane-parallel plage
  models. 
  MC heating becomes visible only higher up as
  chromospheric grain brightening in the \CaII\ \HK\ cores, mostly in
  the network but occasionally above internetwork MCs as the
  ``persistent flasher'' of
  \citetads{1994ASIC..433..251B}.\\ % Brandt++ persistent flasher
  {\em Right:\/} the same sketch served to explain why MCs become
  bright stalks (``faculae'', originally in white light) towards the
  limb. 
  In slanted viewing the fluxtube foot is blocked to higher height by
  the surrounding denser gas (yet higher in the more opaque G band)
  whereas through the relatively empty fluxtube (yet emptier in G-band
  opacity) one views further into the hot = bright granule behind it
  than without a fluxtube crossing the line of sight.
  The apparent stalks represent lack of opacity along that.\\
  {\em Bottom row\/}: the same sketch but modified to illustrate
  1700--1600\,\AA\ MC brightness difference. 
  Outside the tube the 1600\,\AA\ continuum opacity is larger but
  inside it is lower because the neutral metals ionize away (they are
  already minority stage) so that only the scattering Balmer continuum
  and some Rayleigh scattering remain.\\
  {\em Left:\/} at 1600\,\AA\ the MCs are deeper holes than at
  1700\,\AA\ and relatively brighter in byte-scaled top-down images
  (the outside scene is dominated by clapotispheric shocks that
  brighten less or darken). 
  The same apparent deepening from neutral-metal ionization causes the
  classic ``line gap'' phenomenon in \FeI\ lines (\eg\
  \citeads{1991A&A...251..675S}) % Stellmacher+Wiehr moustaches
  which is seen best in \MnI\ lines
  (\citeads{1987ApJ...314..808L}) % Livingston+Wallace
  from lack of microturbulent smearing in surrounding granulation
  (\citeads{2009A&A...499..301V}), % Vitas++ MnI
  and also similar MC ``moustache'' brightening (not EB but pseudo-EB,
  moustaches share that confusion) of the wings of the \NaID\ and
  \MgIb\ minority-stage lines (also
  \citeads{1991A&A...251..675S}). % Stellmacher+Wiehr moustaches
  For an SST/CRISP example of the latter see the MC near the center of
  the small field in \linkadspage{2011A&A...531A..17R}{5}{Figure 4} of
  \citetads{2011A&A...531A..17R}. % Rutten++ NaD1 revgran
  Its brightening enhancement in the wing of the majority-stage \CaIR\
  line in that figure comes from less collisional damping at smaller
  density reducing wing opacities.
  Such wing brightening by less-damping deepening is also seen in
  \Halpha\
  (\citeads{2006A&A...449.1209L}), % Leenaarts++ BPs blue wing Ha
  \Hbeta\ and \CaIIK\
  (\citeads{2006A&A...452L..15L}). % Leenaarts BPs strong-line wings
  For recent SST examples see \linkadspage{2019A&A...631L...5B}{2}{the
  first panels of Fig.~1} of
  \citetads{2019A&A...631L...5B}; % Bose: CaIIK + MgIIk spicules
  less-damping MC brightening is seen particularly well with the
  SST/CHROMIS wide-band filter at 3950\,\AA\ midway between \CaII\ H
  and K.\\ %RR link?
  {\em Right:\/} towards the limb the MCs have higher-up dark foot
  blocking at 1600\,\AA\ by the more opaque surroundings, but the view
  through the tube deep into the hot granule behind starts deeper down
  at 1600\,\AA\ and extends further out in reaching $\tau_\mu \tis\ 1$
  than at 1700\,\AA. 
  The 1600\,\AA\ stalk therefore differs in morphology from the
  1700\,\AA\ stalk, being brighter with apparent limbward shifts
  utterly evident in \rrref{figure}{fig:tileshifts-1617-0}.
  }\end{figure*}
%===========================================================================

%% appendix Halpha-304
 
% fig:scatha304
%===========================================================================
\begin{figure*}
  \centering
  \includegraphics[width=0.33\textwidth]{\deffigs/scatha304}
  \hspace{-1mm}
  \includegraphics[width=0.33\textwidth]{\deffigs/scatmeanha304}
  \hspace{-1mm}
  \includegraphics[width=0.33\textwidth]{\deffigs/scat304131}
%%  \includegraphics[width=0.35\textwidth]{\deffigs/scatmeanhaprod}
  \caption[Strous diagrams]
  {\label{fig:scats} %
  \addtocline{Appendix B}
  Strous scatter diagrams.  
  The format and inserted numbers are explained in
  \linkadspage{2019A&A...632A..96R}{2}{Section~2} of
  \citetads{2019A&A...632A..96R} % Rutten+Rouppe+DPontieu rbecontrails
  with \linkadspage{2019A&A...632A..96R}{7}{Figure~5 there} a
  relatively easy to interpret example. 
  I make Strous diagrams with
  \href{https://webspace.science.uu.nl/~rutte101/rridl/cubelib/scatcont.pro}
  {\tt scatcont.pro} based on
  \href{https://webspace.science.uu.nl/~rutte101/rridl/collib/scatter_aw.pro}
  {Alfred de Wijn's version}.\\
%%  (the curved dashing came from Harold de Wijn).\\
  {\em First panel:\/}  AIA\,\,304\,\AA\ against GONG \Halpha.
  For AIA\,\,304\,\AA\ the temporal average of the
  15-min sequence is used, for \Halpha\ the non-reversed GONG image of
  \rrref{figure}{fig:fieldha} blurred over 30 pixels. 
  The apparent overall correspondence of the grey patches in
  \rrref{figures}{fig:fieldharev} and \ref{fig:field304} is quantified
  as the significant downward tilt of the contour mountain of which
  the extended summit corresponds to grey in the images. 
  Without correlation the mountain would be round with perpendicular
  first-moment curves.
  The rightward tilt of the upper end of the vertical first-moment
  curve suggests slightly brighter than normal grey for \Halpha\ at
  brushfire sites.\\
  % This diagram might be improved by downloading and averaging the
  % other GONG images taken during this SDO sequence duration, but it
  % seems better to perform such \Halpha\ -- \HeII\,304\,\AA\
  % comparisons with higher-quality data.\\
  {\em Second panel:\/} similar but now using sequence-averaged GONG
  \Halpha.  
  My success in co-aligning the single reversed \Halpha\ image of
  \rrref{figure}{fig:fieldharev} with the AIA\,304\,\AA\ image of
  \rrref{figure}{fig:field304} made me develop
  \href{https://webspace.science.uu.nl/~rutte101/rridl/gonglib/gong_sdo.pro}
  {\tt gong\_sdo.pro} to co-align each of the best in a sequence of
  GONG \Halpha\ images with simultaneous AIA\,304\,\AA\ images. 
  My motivation was that this may serve to co-align any \Halpha\
  observation with SDO by using GONG \Halpha\ as intermediary, and
  also look-alike scenes such as ALMA images. 
  Because the GONG images vary much in quality and considerably in
  scale, position and orientation automating such co-alignment is
  non-trivial, but I succeeded in obtaining a co-aligned GONG \Halpha\
  sequence for the present SDO downloads.   
  The resulting Strous diagram is similar to the one at left but shows
  tighter relationships due to the now dual 15-min temporal and 30-px
  spatial averaging.
  This improvement fits my view of the chromosphere: heating to AIA
  304\,\AA\ visibility occurs momentarily in the tips of spicules-II
  followed by darkening \Halpha-core fibrils along their tracks,
  darkest at the track onsets so that the correlation concerns fine
  structures that are not precisely synchronous nor co-spatial but
  closely adjacent in space and time.  
  Again, the tilted scatter mountain describes the grey chromospheric
  patches seen ubiquitously everywhere whereas the brightest 304\,\AA\
  pixels describe fires. 
  These appear only slightly brighter than average in \Halpha\ so that
  low-resolution \Halpha\ does not offer a viable means to locate them.\\
  {\em Third panel\/}: AIA\,131 against 304\,\AA, showing yet tighter
  spatial correlation for most-common grey pixels in
  \rrref{figures}{fig:field304} and \ref{fig:field131}. 
  For both sequences the temporal means are used.
  I was curious about the small North-ward promontory on the North
  coast of this contour island. 
  Inspection with {\tt showex}, which can plot Strous diagrams live
  while blinking and also offers box-selection with image pixel
  coloring, made me add the green and blue selection boxes. 
  Their pixels are colored correspondingly in
  \rrref{figure}{fig:sdoroiloc131}. 
  The blue ones appear to represent a viable fire locator and so
  inspired the multiplicative fire detector tested and described in
  \rrref{figure}{fig:sdoroiloc304x131}. 
  It serves as triple member in
  \rrref{figures}{fig:sdo-minx-193}--\ref{fig:sdo-sp-min-mag} to
  separate chromospheric and coronal heating.
  }\end{figure*}
%===========================================================================


% fig:drifts
%===========================================================================
\begin{figure*}
  \centering
  \includegraphics[width=0.49\textwidth]{\deffigs/shifts_304-mag}
  \includegraphics[width=0.49\textwidth]{\deffigs/check_xal_131-304}
  \caption[SDO cross-alignment results]
  {\label{fig:drifts}%
  {\em Left\/}: standard {\tt driftscenter} plot from the SDO
  cross-alignment pipeline for the present SDO download, for the AIA
  304\,\AA\ versus HMI magnetogram pair.
  These are made from low-cadence 700$\times$700 arcsec$^2$ center
  cutouts by tiling into 30$\times$30~arcsec$^2$ subfields as in
  \rrref{figures}{fig:tileshifts-1617-0} and
  \ref{fig:tileshifts-1617-220} and for every time step determining
  and averaging spatial offsets by cross-correlation per tile pair,
  after appropriate image ``mucking'' in
  \href{https://webspace.science.uu.nl/~rutte101/rridl/sdolib/sdo_muckimagepair.pro}
  {\tt sdo\_muckimagepair.pro} to make them appear more similar and
  using {\tt heightdiff} correction, here with limb value 3600~km
  determined from zonal tile-shift averaging as in
  \rrref{figure}{fig:zonalshifts-1617-0}. 
  The error bars are 96\% confidence limits for the next tile sample
  per time step.
  Their average values are specified at lower left.
  The boxed samples are outliers removed in iterative spline fitting.  
  The resulting spline curves are stored and used to cross-align the
  actual target data. 
  Their 1$\sigma$ reliability is specified at the lower right.
  The pipeline produces such graphs for all pairs it employs. 
  Generally they show time-varying drifts up to a few pixels between
  SDO diagnostics (more after eclipses or hiccups). 
  % These offsets improved when the AIA software engineers moved the
  % database last year from once-per-week to every-3-hours limb fitting
  % used by SSW's {\tt aia\_prep.pro}, but the drifts are often faster
  % and I usually find offsets up to about 2~px.
  %RR maybe they are better now but I use no MPO lookup for (X,Y) 
  Fixing the EUVs to HMI or UV is the hardest; currently this
  304\,\AA\ -- magnetogram pair is my default anchor choice.\\
  {\em Right\/}: {\tt driftscenter} check plot after all
  cross-alignments for the AIA 131\,\AA\ versus 304\,\AA\ pair, also
  made with
  \href{https://webspace.science.uu.nl/~rutte101/rridl/sdolib/sdo_writepairspline.pro}
  {\tt sdo\_writepairspline,pro}. 
  The vertical axis range is smaller.
  Currently, the pipeline does not cross-align these directly but it
  roundabout cross-aligns 211\,\AA\ to 304\,\AA, 335\,\AA\ to
  211\,\AA, 131\,\AA\ to 335\,\AA. 
  There are more such chained cross-alignments, all anchored to the
  304\,\AA\ to HMI magnetogram alignment at left, with their orders
  defined in
  \href{https://webspace.science.uu.nl/~rutte101/rridl/sdolib/
  sdo_getsumsplineshift.pro}{\tt sdo\_getsumsplineshift.pro} from {\tt
  showex} scene comparisons to select best-matching pairs as well as
  appropriate mucking.
  Remaining errors add up statistically in such multi-step chains. 
  Here, this check from cross-aligning the pipeline disk-center
  results, not its input, shows that the final errors for this pair
  are negligible, fully so at best-match time (14:58:46~UT). 
  Before cross-alignment this {\tt aia\_prepped} input pair had
  consistent $(\Delta x,\Delta y) \approx (+0.3,-1.1)$~px offsets.
  Their reduction to 0.1~px ensures that the fire detector of
  \rrref{figure}{fig:sdoroiloc304x131} multiplies appropriate pixel
  pairs.
  }\end{figure*}
%===========================================================================


